Arc-Standard Spinal Parsing with Stack-LSTMs

We present a neural transition-based parser for spinal trees, a dependency representation of constituent trees. The parser uses Stack-LSTMs that compose constituent nodes with dependency-based derivations. In experiments, we show that this model adapts to different styles of dependency relations, but this choice has little effect for predicting constituent structure, suggesting that LSTMs induce useful states by themselves.

==> dev-fulltable.tex <==
\begin{table}
\begin{tabular}{|lccccc|}
\hline
 & \multicolumn{3}{c}{Constituents} & SD & YM \\
      & LR    & LP    & F1    & UAS   & UAS\\
\hline
Left  & 91.18 & 90.93 & 91.05 & -     & - \\
%
%MODEL out-v4/mod-v4-right-s-dev-2.der
%Bracketing Recall         =  91.03
%Bracketing Precision      =  91.20
%Bracketing FMeasure       =  91.11
Right & 91.03 & 91.20 & 91.11 & - & - \\
%
%MODEL out-v4/mod-v4-sd-r-dev-1.der
%Bracketing Recall         =  90.56
%Bracketing Precision      =  90.84
%Bracketing FMeasure       =  90.70
SD-r & 90.56 & 90.84 & 90.70 & 93.50  & - \\
% 
%SD-sr & 90.50 & 90.89 & 90.69 & 93.43 & - \\
%
%MODEL out-v4/mod-v4-sd-s-dev-2.der
%Bracketing Recall         =  90.75
%Bracketing Precision      =  91.11
%Bracketing FMeasure       =  90.93
%Complete match            =  42.73
%Tagging accuracy          =  96.77
%Unlabeled attachment score: 33140 / 35446 * 100 = 93.49 %
SD-s  & 90.75 & 91.11 & 90.93 & 93.49 & - \\
% (v3)
%SD-s  & 90.74 & 90.75 & 90.74 & 93.25 & - \\
% (v3)
SD-X  & -     & -     & -     & 93.30 & - \\
%
%
%
% (v3)
%YM-sr & 90.03 & 90.67 & 90.35 & -     & 93.05 \\
% MODEL out-v4/mod-v4-ym-r-dev-2.der
%Bracketing Recall         =  90.24
%Bracketing Precision      =  91.13
%Bracketing FMeasure       =  90.68
%Complete match            =  40.44
% YM Unlabeled attachment score: 33016 / 35446 * 100 = 93.14 %
YM-r  & 90.24 & 91.13 & 90.68 & -    & 93.14 \\
%
% (v3)
%YM-s  & 90.60 & 91.01 & 90.80 & -     & 93.03 \\				
%MODEL out-v4/mod-v4-ym-s-dev-2.der
%Bracketing Recall         =  90.82
%Bracketing Precision      =  90.84
%Bracketing FMeasure       =  90.83
%Complete match            =  42.08
%YM Unlabeled attachment score: 32973 / 35446 * 100 = 93.02 %
YM-s & 90.82 & 90.84 & 90.83 & -   & 93.02 \\
%
% (v3)
%YM-X  & -     & -     & -     & - 	  & 92.93 \\				
%MODEL out-v4/mod-v4-ym-x-dev-2.der
% YM Unlabeled attachment score: 32961 / 35446 * 100 = 92.99 %
YM-X & - & - & - & - & 92.99 \\
%
\hline
\end{tabular}
\caption{Constutuency and Dependency Results on the PTB development set.}
\end{table}


